Visibility-Aware RRT* for Safety-Critical Navigation of Perception-Limited Robots in Unknown Environments

Safe autonomous navigation in unknown environments remains a critical challenge for robots with limited sensing capabilities. While safety-critical control techniques, such as Control Barrier Functions (CBFs), have been proposed to ensure safety, their effectiveness relies on the assumption that the robot has complete knowledge of its surroundings. In reality, robots often operate with restricted field-of-view and finite sensing range, which can lead to collisions with unknown obstacles if the planner is agnostic to these limitations. To address this issue, we introduce the Visibility-Aware RRT* algorithm that combines sampling-based planning with CBFs to generate safe and efficient global reference paths in partially unknown environments. The algorithm incorporates a collision avoidance CBF and a novel visibility CBF, which guarantees that the robot remains within locally collision-free regions, enabling timely detection and avoidance of unknown obstacles. We conduct extensive experiments interfacing the path planners with two different safety-critical controllers, wherein our method outperforms all other compared baselines across both safety and efficiency aspects.

==> _II.Preliminaries/b_lqr.tex <==
Linear Quadratic Regulator (LQR) computes optimal control policies for linear systems, and can be applied to nonlinear systems by linearizing the system around an operating point $(\vx_o, \vu_o)$, i.e., taking the first-order Taylor expansion of a nonlinear dynamics $F$ around this point:
\begin{equation}
\dot{\vx} \approx F(\vx_o, \vu_o) + A\bar{\vx} + B\bar{\vu},
\label{eq:linearize_dynamics}
\end{equation}
where $\bar{\vx} = \vx - \vx_o$, $\bar{\vu} = \vu - \vu_o$, $A = \frac{\partial F}{\partial \vx}|_{(\vx_o, \vu_o)}$, $B = \frac{\partial F}{\partial \vu}|_{(\vx_o, \vu_o)}$. Given an infinite time horizon cost function:
\begin{equation}
J= \int_{0}^{\infty} ( \, \bar{\vx}^\top Q \bar{\vx} + \bar{\vu}^\top R \bar{\vu} \, ) \, \mathrm{d}t,
\label{eq:lqr_cost}
\end{equation}
where $Q = Q^\top \succeq 0$ and $R = R^\top \succ 0$ are weight matrices, one can compute the locally optimal control policy $\calK_{\text{lqr}}^*(\vx) = -K_{\text{lqr}} \vx$ by solving the algebraic Riccati equation:
\begin{equation}
A^\top P + PA - PBR^{-1}B^\top P + Q = 0.
\label{eq:riccatti}
\end{equation}
Solving~\eqref{eq:riccatti} for $P$, the LQR gain matrix is: 
\begin{equation}
K_{\text{lqr}} = R^{-1}B^\top P.
\label{eq:lqr_gain}
\end{equation}

